On the JI-RADAR: Uncovering Sustainability Tool Support for Requirements Engineering

Context: Software-intensive systems are integral to nearly all facets of modern society [1]. Consequently, both their sustainability and their role in facilitating sustainable processes must be established by design [2], [3]. Software sustainability is defined as "the preservation of the long-term and beneficial use of software, and its appropriate evolution, in a context that continuously changes" [2]. RE Problem & Motivation: Regulatory initiatives increasingly require (software) organizations to integrate sustainability into their day-to-day business and operational processes. The United Nations 2030 Agenda formulated 17 Sustainable Development Goals (SDGs) [6], while the EU passed the Corporate Sustainability Reporting Directive (CSRD), which requires companies to publish and audit sustainability-related information [7]. Regulations and laws require organizations in the software development sector to disclose both qualitative and quantitative sustainability metrics, among other obligations [1]. Consequently, integrating sustainability reporting processes into the software development life cycle becomes increasingly important. RE processes often lack systematic methods to elicit, analyze, and prioritize sustainability requirements alongside functional and non-functional requirements, and studies indicate that tool support for this integration remains limited [4]. To address this gap, we introduce JI-RADAR, which supports stakeholders involved in system design (e.g., developers, requirements engineers, project managers, and usability engineers) [5] by providing practical tools to integrate sustainability into the RE process. We extend the widely used Atlassian Jira platform [8] by implementing a ready-to-use plugin that can be directly adopted in industrial practice.

==> _format.tex <==
\usepackage{fancyhdr}
\usepackage{amsthm}%
\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
\usepackage{manyfoot}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{amsmath,amssymb,amsfonts} %%assymb breaks the acm template
\usepackage{url}
\usepackage{booktabs} % For formal tables                  
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{hyperref}
\usepackage{balance}
\usepackage{tabularx}

\usepackage{booktabs}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{caption}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{float}
\usepackage[shortlabels]{enumitem}
\usepackage[font=small]{caption}

\usepackage{wasysym}

\usepackage{csquotes}
\MakeOuterQuote{"}

\definecolor{commentGreen}{RGB}{128,127,41}
\definecolor{stringGreen}{RGB}{0,127,38}
\definecolor{keywordRed}{RGB}{151,0,11}
\definecolor{typePurple}{RGB}{128,3,82}
\definecolor{variableBlue}{RGB}{0,0,255}
\definecolor{annotationRed}{RGB}{198,4,38}
\definecolor{annotationBlue}{RGB}{32,21,223}

\newcommand{\etal}[1][]{%
\ifthenelse{\equal{#1}{}}{\emph{et~al.}\xspace}{\emph{et~al.}~\cite{#1}\xspace}%
}

\newcommand{\citesec}[1]{Section~\ref{sec:#1}}
\newcommand{\citefig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\citealgo}[1]{\textsc{Listing}~\ref{algo:#1}}
\newcommand{\citelisting}[1]{\textsc{Listing}~\ref{lst:#1}}
\newcommand{\citetable}[1]{{Table}~\ref{tab:#1}}
\newcommand{\citedef}[1]{\textsc{Definition}~\ref{def:#1}}
\newcommand{\citesecs}[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}

% \newcommand{\mv}[1]{{\textcolor{orange}{#1}}}%orange
% \newcommand{\ig}[1]{{\textcolor{blue}{#1}}}%blue
% \newcommand{\ta}[1]{{\textcolor{green}{#1}}}%green

% \newcommand{\fwname}{{\textcolor{purple} EduComp}\xspace}%orange


\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash}p{#1}} 


\newcommand{\bullitem}[1]{\noindent$\bullet$\textbf{ #1}}

\newcommand{\intqte}[1]{\emph{#1}}

